FedRand: Enhancing Privacy in Federated Learning with Randomized LoRA Subparameter Updates

Federated Learning (FL) is a widely used framework for training models in a decentralized manner, ensuring that the central server does not have direct access to data from local clients. However, this approach may still fail to fully preserve data privacy, as models from local clients are exposed to the central server during the aggregation process. This issue becomes even more critical when training vision-language models (VLMs) with FL, as VLMs can easily memorize training data instances, making them vulnerable to membership inference attacks (MIAs). To address this challenge, we propose the FedRand framework, which avoids disclosing the full set of client parameters. In this framework, each client randomly selects subparameters of Low-Rank Adaptation (LoRA) from the server and keeps the remaining counterparts of the LoRA weights as private parameters. After training both parameters on the client's private dataset, only the non-private client parameters are sent back to the server for aggregation. This approach mitigates the risk of exposing client-side VLM parameters, thereby enhancing data privacy. We empirically validate that FedRand improves robustness against MIAs compared to relevant baselines while achieving accuracy comparable to methods that communicate full LoRA parameters across several benchmark datasets.

==> preamble/biblatex.tex <==
\usepackage[
    natbib=true,
    style=authoryear,
    backref=true,
    uniquelist=false,
    sorting=nyt,
    maxcitenames=2,
    mincitenames=1,
    maxbibnames=100,
    minbibnames=100,
]{biblatex}

\renewbibmacro*{pageref}{%
  \iflistundef{pageref}
    {}
    {\printtext[parens]{\printlist{pageref}}}}

\setlength{\bibitemsep}{1.0em}

\DeclareFieldFormat{in}{} % Suppress "In:" in references
\DeclareFieldFormat{citehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}%
  \bibhyperref{#1}
}
\DeclareFieldFormat{textcitehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}%
  \bibhyperref{%
    #1%
    \ifbool{cbx:parens}
      {\bibcloseparen\global\boolfalse{cbx:parens}}
      {}}}

\savebibmacro{cite}
\savebibmacro{textcite}

\renewbibmacro*{cite}{%
  \printtext[citehyperref]{%
    \restorebibmacro{cite}%
    \usebibmacro{cite}}}

\renewbibmacro*{textcite}{%
  \ifboolexpr{
    ( not test {\iffieldundef{prenote}} and
      test {\ifnumequal{\value{citecount}}{1}} )
    or
    ( not test {\iffieldundef{postnote}} and
      test {\ifnumequal{\value{citecount}}{\value{citetotal}}} )
  }
    {\DeclareFieldAlias{textcitehyperref}{noformat}}
    {}%
  \printtext[textcitehyperref]{%
    \restorebibmacro{textcite}%
    \usebibmacro{textcite}}}

\newcommand{\neuripsbooktitle}[1]{%
  Advances in Neural Information Processing Systems  (NeurIPS)
}

\newcommand{\ordinalsuffix}[1]{%
  \ifcase#1 th% 0
  \or st% 1
  \or nd% 2
  \or rd% 3
  \else th% 4–9
  \fi
}

\newcommand{\icmlbooktitle}[1]{%
  International Conference on Machine Learning (ICML)%
}

\newcommand{\aistatsbooktitle}[1]{%
  International Conference on Artificial Intelligence and Statistics (AISTATS)%
}

\newcommand{\iclrbooktitle}[1]{%
  International Conference on Learning Representations (ICLR)%
}

\newcommand{\cvprbooktitle}[1]{%
  Conference on Computer Vision and Pattern Recognition (CVPR)%
}


% % Suppress "In:" from references
% \renewbibmacro{in:}{%
%   \ifentrytype{article}{}{}% Don't include "In:" for any entry
% }



\addbibresource{references.bib}
% Custom bibliography driver for "article"
\DeclareBibliographyDriver{inproceedings}{%
  \printnames{author}% Print authors
  \newunit\newblock
  \printfield{title}% Print title
  \newunit\newblock
  \printfield{booktitle}% Print journal name
  \setunit{\addcomma\space}% Add a comma and space after journal
  \printfield{year}% Print year
  \adddot% Add a period after the year
  \newunit\newblock
  \usebibmacro{pageref}% Include backreferences
  \finentry% End entry
}


\DeclareBibliographyDriver{misc}{%
  \printnames{author}% Print authors
  \newunit\newblock
  \printfield{title}% Print title
  \newunit\newblock
  \printfield{url}% Print journal name
  \setunit{\addcomma\space}% Add a comma and space after journal
  \printfield{year}% Print year
  \adddot% Add a period after the year
  \newunit\newblock
  \usebibmacro{pageref}% Include backreferences
  \finentry% End entry
}

\DeclareFieldFormat{citehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}%
  \bibhyperref{#1}% Ensure no trailing spaces
}

\DeclareFieldFormat{textcitehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}%
  \bibhyperref{%
    #1% Ensure no trailing spaces
    \ifbool{cbx:parens}
      {\bibcloseparen\global\boolfalse{cbx:parens}}
      {}}%
}

% Custom formatting for year
\DeclareFieldFormat{year}{#1} % Suppress any extra space



\renewbibmacro*{pageref}{%
  \iflistundef{pageref}
    {}
    {\printtext[parens]{cit. on p.~\printlist[pageref]{pageref}}}}

==> tables/mia_delta.tex <==
\begin{table}[th]
\centering
\caption{MIA-delta}
\label{tab:mia-delta}
\resizebox{0.48\textwidth}{!}{\begin{tabular}{lcccc}
 \toprule
 & \multicolumn{2}{c}{\textbf{Rényi Entropy Max\_0\%} ($\downarrow$)} & \multicolumn{2}{c}{\textbf{Rényi Entropy Max\_10\%} ($\downarrow)$}  \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
 & image &  caption &  image &  caption  \\
\midrule
FedAvg (server)  & 49.96 & 70.22 & \underline{54.57} & 70.22   \\
FedAvg (client) & 51.68 & 70.68 & 54.71 & 70.69 \\
FedPer (2 layer) & 50.73 & 70.01 & 56.76 & 70.03 \\
FedPer (4 layer) &  51.77 & 69.71 & 57.74 & 69.73 \\
FedPara & 53.48 & 69.67 & 57.07 & 69.63  \\
\midrule
\textbf{FedRand (server)} & \underline{48.90} & \textbf{67.02} & \textbf{53.84} & \textbf{66.61} \\
\textbf{FedRand (client)} & \textbf{47.83} & \underline{68.51} & 54.99 & \underline{68.51} \\
\bottomrule
\end{tabular}
}
\end{table}

